How to Catch $k$ Grid Points

Given a positive integer $k$, we study the problem of finding a convex polygon of minimum perimeter that encloses exactly $k$ points of $\mathbf{Z}^2$. We show that an optimal polygon is contained in a circular annulus of width $O(k^{1/6})$, has $\Theta(k^{1/3})$ boundary grid points, and its longest edge has length $\Theta(k^{1/4})$. Using these structural bounds, we present a deterministic algorithm that computes an optimal polygon in $O(k^{29/18+o(1)})$ time, improving over the previous $O(k^3)$-time algorithm.

==> figs/rt_table.tex <==
%
  \centering
  \small
  \begin{tabular}[t]{rr}
    \toprule
    $k$ Value & Time (s) \\
    \midrule
    10 & 0.03 \\
    20 & 0.02 \\
    50 & 0.02 \\
    100 & 0.03 \\
    500 & 0.05 \\
    1,000 & 0.09 \\
    5,000 & 0.83 \\
    10,000 & 3.61 \\
    \bottomrule
  \end{tabular}
  \hfill
  \begin{tabular}[t]{rr}
    \toprule
    $k$ Value & Time (s) \\
    \midrule
    20,000 & 10.14 \\
    30,000 & 18.98 \\
    40,000 & 42.61 \\
    50,000 & 46.30 \\
    60,000 & 73.37 \\
    70,000 & 99.33 \\
    80,000 & 117.15 \\
    90,000 & 130.22 \\
    \bottomrule
  \end{tabular}
  \hfill
  \begin{tabular}[t]{rr}
    \toprule
    $k$ Value & Time (s) \\
    \midrule
    100,000 & 131.60 \\
    150,000 & 385.86 \\
    200,000 & 556.94 \\
    250,000 & 947.47 \\
    300,000 & 1,214.20 \\
    350,000 & 1,525.66 \\
    1,500,000 & 4,716.69 \\
    2,500,000 & 6,827.01 \\
    \bottomrule
  \end{tabular}

